Financial Crime & Fraud Detection Using Graph Computing: Application Considerations & Outlook

In recent years, the unprecedented growth in digital payments fueled consequential changes in fraud and financial crimes. In this new landscape, traditional fraud detection approaches such as rule-based engines have largely become ineffective. AI and machine learning solutions using graph computing principles have gained significant interest. Graph neural networks and emerging adaptive solutions provide compelling opportunities for the future of fraud and financial crime detection. However, implementing the graph-based solutions in financial transaction processing systems has brought numerous obstacles and application considerations to light. In this paper, we overview the latest trends in the financial crimes landscape and discuss the implementation difficulties current and emerging graph solutions face. We argue that the application demands and implementation challenges provide key insights in developing effective solutions.

==> Makefile <==
MAIN=main
BIB=bib
OUTPUT_DIR=output
AUX_DIR=output_aux

.PHONY: all check link clean travis data tatoeba

pdf:
	latexmk -pdf $(MAIN) -auxdir=$(OUTPUT_DIR) -outdir=$(OUTPUT_DIR)

all: pdf
	make -C code/programs

check:
	chktex -n1 -n2 -n3 -n8 -n11 -n12 -n13 -n14 -n26 -n34 -n33 -n36 -n40 -n44 $(MAIN)
	biber --tool -V $(BIB).bib
	rm -f $(BIB)_bibertool.bib

lint:
	biber --tool $(BIB).bib --output-fieldcase=lower --isbn-normalise
	mv $(BIB)_bibertool.bib $(BIB).bib

arxiv: pdf
	mkdir -p arxiv
	cp *.pdf $(OUTPUT_DIR)/*.bbl *.bib *.tex *.cls *.bst arxiv
	#Download any new versions of packages here
	#e.g.
	#curl -L -o arxiv/algorithm2e.sty https://ctan.sharelatex.com/tex-archive/macros/latex/contrib/algorithm2e/tex/algorithm2e.sty
	#Test build
	cd arxiv && latexmk -pdf $(MAIN) -auxdir=arxivtest -outdir=arxivtest && rm -rf arxivtest
	cd arxiv && zip arxiv.zip *

clean:
	latexmk -c -pdf
	rm -rvf *.bbl *.blg *.aux *.fls *.fdb_latexmk *.log *.out *.toc $(MAIN).pdf $(AUX_DIR) $(OUTPUT_DIR) arxiv

travis:
	#Old latexmk doesn't understand auxdir and outdir options
	latexmk -pdf -pdflatex='pdflatex %S %O -interaction=nonstopmode -halt-on-error' $(MAIN)

######################
# Download data
######################
TATOEBA_CORPUS = data/tatoeba/users_sentences.csv \
	data/tatoeba/user_languages.csv \
data/tatoeba/sentences_in_lists.csv \
data/tatoeba/links.csv \
data/tatoeba/tags.csv \
data/tatoeba/sentences_detailed.csv \
data/tatoeba/user_lists.csv

data: $(TATOEBA_CORPUS)

tatoeba: $(TATOEBA_CORPUS)

data/tatoeba/users_sentences.csv:
	curl --create-dirs -R -L -z $@ -o $@ https://downloads.tatoeba.org/exports/users_sentences.csv

data/tatoeba/%.csv: data/tatoeba/%.tar.bz2
	tar -xjvf $< -C data/tatoeba

data/tatoeba/%.tar.bz2:
	curl --create-dirs -R -L -z $@ -o $@ https://downloads.tatoeba.org/exports/$(notdir $@)


